Lyapunov stabilization of a nonlocal LWR traffic flow model

Using a nonlocal macroscopic LWR-type traffic flow model, we present an approach to control the nonlocal velocity towards a given equilibrium velocity. Therefore, we present a Lyapunov function measuring the $L^2$ distance between these velocities. We compute the explicit rate at which the system tends towards the stationary speed. The traffic is controlled by a leading vehicle. Numerical examples demonstrate the theoretical results and possible extensions of them.

==> macros.tex <==
\usepackage[english]{babel}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{a4wide}
\usepackage{verbatim}
\RequirePackage{ifthen}
\RequirePackage[T1]{fontenc}
\RequirePackage{amsthm}
\RequirePackage{color}
\RequirePackage{listings} 
\RequirePackage{epstopdf}
\RequirePackage{emptypage}
\RequirePackage[nolist]{acronym}
\RequirePackage{multirow}
\RequirePackage{enumerate,enumitem}
\RequirePackage{caption}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta}
\RequirePackage{latexsym,amscd,makeidx}
\RequirePackage{exscale}
\RequirePackage{mathrsfs}
\RequirePackage{hyperref}
\RequirePackage{url}
\RequirePackage{booktabs}
\RequirePackage{esdiff}
\RequirePackage{listings}
\RequirePackage{tabularx}
%\RequirePackage[numbers]{natbib}
\RequirePackage{verbatim}
\RequirePackage{comment}
%\RequirePackage{cite}
\RequirePackage{cleveref}
\crefname{equation}{}{}
\Crefname{Equation}{}{}
\usepackage{pgfplots} 
\usepackage{pgfgantt}
\usepackage{pdflscape}
%\usepackage[notref,notcite]{showkeys}
\pgfplotsset{compat=newest} 
\pgfplotsset{plot coordinates/math parser=false}
\numberwithin{equation}{section}
% Switch: Hide or show comments
	\newif\ifshowcomments								
%	\showcommentstrue				% show comments
	\showcommentsfalse				% hide comments


% Definition of environments
	\definecolor{mygrey}{gray}{0.65}
	
	% Detailed comments
	\ifshowcomments
		% Display comments in a specified environment
		\newenvironment{bcomment}[1][]
	 	{~\\~\\ \begin{color}{mygrey}\begin{small}\noindent\textbf{COMMENT: #1}~\\}
	 	{\end{small}\end{color}~\\~\\}
	\else
		% Hide comments
	 	\excludecomment{bcomment}
	\fi
	% Inline-Comments
	
	\ifshowcomments
		\newcommand{\scomment}[1]{{\color{mygrey} [#1]}}  % small comments within lines
	\else
		\newcommand{\scomment}[1]{\iffalse #1 \fi}
	\fi

% Adjust sign of a number for the tikz picture of the grid 
	\newcommand\checkindex[1]{
		\pgfmathsetmacro{\var}{#1}
		\pgfmathparse{ifthenelse(\var==0, "",ifthenelse(\var>0, "+#1","#1"))} \pgfmathresult}%

%For tikz plots
\newlength\fwidth

% Create 'todo' marker (called by \todo{TEXT})
\newcommand{\margtodo}
{\marginpar{\textbf{\textcolor{red}{ToDo}}}{}}
\newcommand{\todo}[1]
{{\textbf{\textcolor{red}{-- \margtodo{}#1 --}}}{}}

\newcommand{\margidea}
{\marginpar{\textbf{\textcolor{orange}{Idea}}}{}}
\newcommand{\idea}[1]
{{\textbf{\textcolor{orange}{-- \margidea{}#1 --}}}{}}

\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\BV}{BV}

\theoremstyle{plain}						% Default
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

%%%Notation:
%Define some shortcuts
%% math calligraphy
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%% math blackboard bold
%\newcommand{\A}{\mathbb{A}}
%\newcommand{\B}{\mathbb{B}}
%\newcommand{\C}{\mathbb{C}}
%\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
%\newcommand{\I}{\mathbb{I}}
%\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
%\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\T}{\mathbb{T}}
%\newcommand{\U}{\mathbb{U}}
%\newcommand{\V}{\mathbb{V}}
%\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}

%% New commands
\newcommand{\OAP}{$(\Omega,\mathcal{A},P)$}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
\newcommand{\sign}{\operatorname{sgn}}
\newcommand{\Div}{\operatorname{div}}
\newcommand{\lano}{\mathrm{o}}
\newcommand{\lanO}{\mathrm{O}}
\newcommand{\dint}{\displaystyle\int}
\newcommand{\dsup}{\displaystyle\sup}
\newcommand{\dsum}{\displaystyle\sum}
%\newcommand{\BV}{\operatorname{BV}}
\newcommand{\TV}{\operatorname{TV}}
%System
\newcommand{\consys}{\cQ}

%Indicies
\newcommand\half{{\frac12}}
\newcommand\jmo{{j-1}}
\newcommand\jmh{{j-\half}}
\newcommand\jpmh{{j\pm\half}}
\newcommand\jph{{j+\half}}
\newcommand\jpo{{j+1}}
\newcommand{\jpk}{{j+k}}
\newcommand{\jpko}{{j+k+1}}
\newcommand{\kmo}{{k-1}}
\newcommand\npo{{n+1}}

%Step sizes
\newcommand{\Dx}{\Delta x}
\newcommand{\Dt}{\Delta t}

%Computations
\newcommand\dx{\mathit{dx}}
\newcommand\dy{\mathit{dy}}
\newcommand\dt{\mathit{dt}}
\newcommand\ds{\mathit{ds}}
\newcommand{\norm}[1]{{\left\|#1\right\|}}
\newcommand{\abs}[1]{{\left|#1\right|}}

%Spaces:
\newcommand{\LinfR}{{L^\infty(\R)}}
\newcommand{\LinfRR}{{L^\infty(\R;\R)}}
\newcommand{\LoneR}{{L^1(\R)}}
\newcommand{\LoneRR}{{L^1(\R;\R)}}
\renewcommand{\L}[1]{L^{#1}}
\newcommand{\Lloc}[1]{L^{#1}_{loc}}

%Nonlocal look ahead distance for the source term
\newcommand{\nds}{{\nu}}
%Kernel Function for source term
\newcommand{\ws}{W_{\nds}}
%Nonlocal look ahead distance for the transport term
\newcommand{\ndt}{{\eta}}
%Kernel Function for transport term
\newcommand{\wt}{W_{\ndt}}
\newcommand{\twt}{\mathcal{W}_{\ndt}}
%Upperbound for discrete convolution
\newcommand{\Ne}{N_\ndt}

%Kernel Functions transport:
\newcommand{\wtcon}{\wt^{\text{const.}}}
\newcommand{\wtlin}{\wt^{\text{lin.}}}
\newcommand{\wtconcave}{\wt^{\text{conc.}}}
%Coupling function:
\newcommand{\coupling}{g}
\newcommand{\newg}{\Gamma}
%Test functions
\newcommand{\testf}{\phi}

%Discrete rho
\newcommand{\dr}{\rho^{\Dx}}
%N_T Time iterations scheme
\newcommand{\NT}{{N_T}}

%n for different \Dx values for convergence
\newcommand{\nconv}{\mathcal{N}}

%Characteristics
\newcommand{\chr}{X}
%Characteristics of rho, t0, x0
\newcommand{\chrptxz}{{\chr_\rho[t_0,x_0]}}


%Paper Maximum Principle
\renewcommand{\P}{P}
\newcommand{\w}{w}
\newcommand{\coeff}{\mu}
\newcommand\opt{{\text{opt}}}
\newcommand\brho{{\bar\rho}}
\renewcommand{\S}{SI}

% quadrature
\newcommand{\qn}{{\nu}}
\newcommand{\nqn}{{J}}
\newcommand{\qw}{{h}}
\newcommand{\qwn}{\qw_\qn}
\newcommand{\qvar}{{y}}

%Order of reconstruction
\newcommand{\g}{o}
\newcommand{\GPopt}{O}


%For networks
\newcommand{\road}{E}
\newcommand{\roadind}{e}
\newcommand{\vertice}{Z}
\newcommand{\verticeind}{z}
\newcommand{\Ro}{\rho^{\max}_1}
\newcommand{\Rt}{\rho^{\max}_2}
\newcommand{\Rtr}{\rho^{\max}_3}
\newcommand{\Rr}{\rho^{\max}_\roadind}
\newcommand{\po}{\rho_1}
\newcommand{\pt}{\rho_2}
\newcommand{\pe}{\rho_\roadind}
\newcommand{\roadbeginohne}{a}
\newcommand{\roadbegin}{\roadbeginohne_\roadind}
\newcommand{\roadendohne}{b}
\newcommand{\roadend}{\roadendohne_\roadind}
\newcommand{\incoming}{\mathcal{I}}
\newcommand{\incomingind}{i}
\newcommand{\NI}{N_\incoming}
\newcommand{\outgoing}{\mathcal{O}}
\newcommand{\outgoingind}{o}
\newcommand{\NO}{N_\outgoing}
\newcommand{\distMatrix}{\mathbb{A}}
\newcommand{\distpar}{\alpha}
\newcommand{\priopar}{q}
\newcommand{\lipschitzcoupling}{{L_\coupling}}
\newcommand{\totaltraveltime}{TTT}
\newcommand{\outflow}{O}
\newcommand{\congestionmeasure}{CM}


\newcommand{\newgo}{\newg_{\outgoingind}}

%Multilane
\newcommand{\borho}{\boldsymbol{\rho}}
\newcommand{\bodr}{\boldsymbol{\rho}^{\Dx}}
\newcommand{\drl}{\rho^{\Dx,\ell}}
\newcommand{\caratt}[1]{{\chi_{\strut#1}}}
\newcommand{\spt}{\mathop{\rm supp}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\boV}{\boldsymbol{V^\nds}}
%Characteristics of bold rho and \ell
\newcommand{\chrl}{\chr_{\borho,\ell}}
\newcommand{\chrb}{\chr_{\borho}}

%GARZ
%Lagrangian marker
\newcommand{\lm}{\omega}
\newcommand{\vg}{u}
\newcommand{\VG}{U}

\newcommand{\jan}[1]{\textcolor{orange}{[Jan: #1]}}
